Evolving localizations in reaction-diffusion cellular automata

We consider hexagonal cellular automata with immediate cell neighbourhood and three cell-states. Every cell calculates its next state depending on the integral representation of states in its neighbourhood, i.e. how many neighbours are in each one state. We employ evolutionary algorithms to breed local transition functions that support mobile localizations (gliders), and characterize sets of the functions selected in terms of quasi-chemical systems. Analysis of the set of functions evolved allows to speculate that mobile localizations are likely to emerge in the quasi-chemical systems with limited diffusion of one reagent, a small number of molecules is required for amplification of travelling localizations, and reactions leading to stationary localizations involve relatively equal amount of quasi-chemical species. Techniques developed can be applied in cascading signals in nature-inspired spatially extended computing devices, and phenomenological studies and classification of non-linear discrete systems.

==> atex01/01.tex <==
\begin{picture}(32.0,60.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,60.0){\circle*{1.}}
\put(9.6,60.0){\circle*{1.}}
\put(16.0,60.0){\circle*{1.}}
\put(22.4,60.0){\circle*{1.}}
\put(28.800001,60.0){\circle*{1.}}
\put(0.0,54.0){\circle*{1.}}
\put(6.4,54.0){\circle*{1.}}
\put(12.8,54.0){\circle*{1.}}
\put(19.2,54.0){\circle*{1.}}
\put(25.6,54.0){\circle*{1.}}
\put(32.0,54.0){\circle*{1.}}
\put(3.2,48.0){\circle*{1.}}
\put(9.6,48.0){\circle*{1.}}
\put(16.0,48.0){\circle*{1.}}
\put(22.4,48.0){\circle{6.8}}
\put(28.800001,48.0){\circle{6.8}}
\put(0.0,42.0){\circle*{1.}}
\put(6.4,42.0){\circle*{1.}}
\put(12.8,42.0){\circle*{1.}}
\put(19.2,42.0){\circle{6.8}}
\put(25.6,42.0){\circle{6.8}}
\put(32.0,42.0){\circle{6.8}}
\put(3.2,36.0){\circle*{1.}}
\put(9.6,36.0){\circle{6.8}}
\put(16.0,36.0){\circle{6.8}}
\put(22.4,36.0){\circle{6.8}}
\put(28.800001,36.0){\circle{6.8}}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle{6.8}}
\put(12.8,30.0){\circle{6.8}}
\put(19.2,30.0){\circle{6.8}}
\put(25.6,30.0){\circle*{1.}}
\put(32.0,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{1.}}
\put(9.6,24.0){\circle{6.8}}
\put(16.0,24.0){\circle{6.8}}
\put(22.4,24.0){\circle*{1.}}
\put(28.800001,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{1.}}
\put(6.4,18.0){\circle*{1.}}
\put(12.8,18.0){\circle*{1.}}
\put(19.2,18.0){\circle*{1.}}
\put(25.6,18.0){\circle*{1.}}
\put(32.0,18.0){\circle*{1.}}
\put(3.2,12.0){\circle*{1.}}
\put(9.6,12.0){\circle*{1.}}
\put(16.0,12.0){\circle*{1.}}
\put(22.4,12.0){\circle*{1.}}
\put(28.800001,12.0){\circle*{1.}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(19.2,6.0){\circle*{1.}}
\put(25.6,6.0){\circle*{1.}}
\put(32.0,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\put(22.4,0.0){\circle*{1.}}
\put(28.800001,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}









































































































































==> atex01/02.tex <==
\begin{picture}(32.0,60.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,60.0){\circle*{1.}}
\put(9.6,60.0){\circle*{1.}}
\put(16.0,60.0){\circle*{1.}}
\put(22.4,60.0){\circle*{1.}}
\put(28.800001,60.0){\circle*{1.}}
\put(0.0,54.0){\circle*{1.}}
\put(6.4,54.0){\circle*{1.}}
\put(12.8,54.0){\circle*{1.}}
\put(19.2,54.0){\circle*{1.}}
\put(25.6,54.0){\circle*{1.}}
\put(32.0,54.0){\circle*{1.}}
\put(3.2,48.0){\circle*{1.}}
\put(9.6,48.0){\circle*{1.}}
\put(16.0,48.0){\circle*{1.}}
\put(22.4,48.0){\circle*{1.}}
\put(28.800001,48.0){\circle*{1.}}
\put(0.0,42.0){\circle*{1.}}
\put(6.4,42.0){\circle*{1.}}
\put(12.8,42.0){\circle*{6.8}}
\put(19.2,42.0){\circle*{1.}}
\put(25.6,42.0){\circle*{1.}}
\put(32.0,42.0){\circle*{1.}}
\put(3.2,36.0){\circle*{1.}}
\put(9.6,36.0){\circle*{1.}}
\put(16.0,36.0){\circle*{1.}}
\put(22.4,36.0){\circle*{1.}}
\put(28.800001,36.0){\circle*{1.}}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{1.}}
\put(12.8,30.0){\circle*{1.}}
\put(19.2,30.0){\circle*{1.}}
\put(25.6,30.0){\circle*{6.8}}
\put(32.0,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{1.}}
\put(9.6,24.0){\circle*{1.}}
\put(16.0,24.0){\circle*{1.}}
\put(22.4,24.0){\circle*{1.}}
\put(28.800001,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{1.}}
\put(6.4,18.0){\circle*{1.}}
\put(12.8,18.0){\circle*{1.}}
\put(19.2,18.0){\circle*{1.}}
\put(25.6,18.0){\circle*{1.}}
\put(32.0,18.0){\circle*{1.}}
\put(3.2,12.0){\circle*{1.}}
\put(9.6,12.0){\circle*{1.}}
\put(16.0,12.0){\circle*{1.}}
\put(22.4,12.0){\circle*{1.}}
\put(28.800001,12.0){\circle*{1.}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(19.2,6.0){\circle*{1.}}
\put(25.6,6.0){\circle*{1.}}
\put(32.0,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\put(22.4,0.0){\circle*{1.}}
\put(28.800001,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}









































































































































==> atex01/03.tex <==
\begin{picture}(32.0,60.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,60.0){\circle*{1.}}
\put(9.6,60.0){\circle*{1.}}
\put(16.0,60.0){\circle*{1.}}
\put(22.4,60.0){\circle*{1.}}
\put(28.800001,60.0){\circle*{1.}}
\put(0.0,54.0){\circle*{1.}}
\put(6.4,54.0){\circle*{1.}}
\put(12.8,54.0){\circle*{1.}}
\put(19.2,54.0){\circle*{1.}}
\put(25.6,54.0){\circle*{1.}}
\put(32.0,54.0){\circle*{1.}}
\put(3.2,48.0){\circle*{1.}}
\put(9.6,48.0){\circle{6.8}}
\put(16.0,48.0){\circle{6.8}}
\put(22.4,48.0){\circle*{1.}}
\put(28.800001,48.0){\circle*{1.}}
\put(0.0,42.0){\circle*{1.}}
\put(6.4,42.0){\circle{6.8}}
\put(12.8,42.0){\circle{6.8}}
\put(19.2,42.0){\circle{6.8}}
\put(25.6,42.0){\circle*{1.}}
\put(32.0,42.0){\circle*{1.}}
\put(3.2,36.0){\circle*{1.}}
\put(9.6,36.0){\circle{6.8}}
\put(16.0,36.0){\circle{6.8}}
\put(22.4,36.0){\circle{6.8}}
\put(28.800001,36.0){\circle{6.8}}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{1.}}
\put(12.8,30.0){\circle*{1.}}
\put(19.2,30.0){\circle{6.8}}
\put(25.6,30.0){\circle{6.8}}
\put(32.0,30.0){\circle{6.8}}
\put(3.2,24.0){\circle*{1.}}
\put(9.6,24.0){\circle*{1.}}
\put(16.0,24.0){\circle*{1.}}
\put(22.4,24.0){\circle{6.8}}
\put(28.800001,24.0){\circle{6.8}}
\put(0.0,18.0){\circle*{1.}}
\put(6.4,18.0){\circle*{1.}}
\put(12.8,18.0){\circle*{1.}}
\put(19.2,18.0){\circle*{1.}}
\put(25.6,18.0){\circle*{1.}}
\put(32.0,18.0){\circle*{1.}}
\put(3.2,12.0){\circle*{1.}}
\put(9.6,12.0){\circle*{1.}}
\put(16.0,12.0){\circle*{1.}}
\put(22.4,12.0){\circle*{1.}}
\put(28.800001,12.0){\circle*{1.}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(19.2,6.0){\circle*{1.}}
\put(25.6,6.0){\circle*{1.}}
\put(32.0,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\put(22.4,0.0){\circle*{1.}}
\put(28.800001,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}









































































































































==> atex01/04.tex <==
\begin{picture}(32.0,60.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,60.0){\circle*{1.}}
\put(9.6,60.0){\circle*{1.}}
\put(16.0,60.0){\circle*{1.}}
\put(22.4,60.0){\circle*{1.}}
\put(28.800001,60.0){\circle*{1.}}
\put(0.0,54.0){\circle*{1.}}
\put(6.4,54.0){\circle*{1.}}
\put(12.8,54.0){\circle*{1.}}
\put(19.2,54.0){\circle*{1.}}
\put(25.6,54.0){\circle*{1.}}
\put(32.0,54.0){\circle*{1.}}
\put(3.2,48.0){\circle*{1.}}
\put(9.6,48.0){\circle*{1.}}
\put(16.0,48.0){\circle*{1.}}
\put(22.4,48.0){\circle*{1.}}
\put(28.800001,48.0){\circle*{1.}}
\put(0.0,42.0){\circle*{1.}}
\put(6.4,42.0){\circle*{1.}}
\put(12.8,42.0){\circle*{1.}}
\put(19.2,42.0){\circle*{1.}}
\put(25.6,42.0){\circle*{6.8}}
\put(32.0,42.0){\circle*{1.}}
\put(3.2,36.0){\circle*{1.}}
\put(9.6,36.0){\circle*{1.}}
\put(16.0,36.0){\circle*{1.}}
\put(22.4,36.0){\circle*{1.}}
\put(28.800001,36.0){\circle*{1.}}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{1.}}
\put(12.8,30.0){\circle*{6.8}}
\put(19.2,30.0){\circle*{1.}}
\put(25.6,30.0){\circle*{1.}}
\put(32.0,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{1.}}
\put(9.6,24.0){\circle*{1.}}
\put(16.0,24.0){\circle*{1.}}
\put(22.4,24.0){\circle*{1.}}
\put(28.800001,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{1.}}
\put(6.4,18.0){\circle*{1.}}
\put(12.8,18.0){\circle*{1.}}
\put(19.2,18.0){\circle*{1.}}
\put(25.6,18.0){\circle*{1.}}
\put(32.0,18.0){\circle*{1.}}
\put(3.2,12.0){\circle*{1.}}
\put(9.6,12.0){\circle*{1.}}
\put(16.0,12.0){\circle*{1.}}
\put(22.4,12.0){\circle*{1.}}
\put(28.800001,12.0){\circle*{1.}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(19.2,6.0){\circle*{1.}}
\put(25.6,6.0){\circle*{1.}}
\put(32.0,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\put(22.4,0.0){\circle*{1.}}
\put(28.800001,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}









































































































































==> atex01/05.tex <==
\begin{picture}(32.0,60.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,60.0){\circle*{1.}}
\put(9.6,60.0){\circle*{1.}}
\put(16.0,60.0){\circle*{1.}}
\put(22.4,60.0){\circle*{1.}}
\put(28.800001,60.0){\circle*{1.}}
\put(0.0,54.0){\circle*{1.}}
\put(6.4,54.0){\circle*{1.}}
\put(12.8,54.0){\circle*{1.}}
\put(19.2,54.0){\circle*{1.}}
\put(25.6,54.0){\circle*{1.}}
\put(32.0,54.0){\circle*{1.}}
\put(3.2,48.0){\circle*{1.}}
\put(9.6,48.0){\circle*{1.}}
\put(16.0,48.0){\circle*{1.}}
\put(22.4,48.0){\circle{6.8}}
\put(28.800001,48.0){\circle{6.8}}
\put(0.0,42.0){\circle*{1.}}
\put(6.4,42.0){\circle*{1.}}
\put(12.8,42.0){\circle*{1.}}
\put(19.2,42.0){\circle{6.8}}
\put(25.6,42.0){\circle{6.8}}
\put(32.0,42.0){\circle{6.8}}
\put(3.2,36.0){\circle*{1.}}
\put(9.6,36.0){\circle{6.8}}
\put(16.0,36.0){\circle{6.8}}
\put(22.4,36.0){\circle{6.8}}
\put(28.800001,36.0){\circle{6.8}}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle{6.8}}
\put(12.8,30.0){\circle{6.8}}
\put(19.2,30.0){\circle{6.8}}
\put(25.6,30.0){\circle*{1.}}
\put(32.0,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{1.}}
\put(9.6,24.0){\circle{6.8}}
\put(16.0,24.0){\circle{6.8}}
\put(22.4,24.0){\circle*{1.}}
\put(28.800001,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{1.}}
\put(6.4,18.0){\circle*{1.}}
\put(12.8,18.0){\circle*{1.}}
\put(19.2,18.0){\circle*{1.}}
\put(25.6,18.0){\circle*{1.}}
\put(32.0,18.0){\circle*{1.}}
\put(3.2,12.0){\circle*{1.}}
\put(9.6,12.0){\circle*{1.}}
\put(16.0,12.0){\circle*{1.}}
\put(22.4,12.0){\circle*{1.}}
\put(28.800001,12.0){\circle*{1.}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(19.2,6.0){\circle*{1.}}
\put(25.6,6.0){\circle*{1.}}
\put(32.0,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\put(22.4,0.0){\circle*{1.}}
\put(28.800001,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}









































































































































==> atex02/03.tex <==
\begin{picture}(32.0,60.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,60.0){\circle*{1.}}
\put(6.4,60.0){\circle*{1.}}
\put(12.8,60.0){\circle*{1.}}
\put(19.2,60.0){\circle*{1.}}
\put(25.6,60.0){\circle*{1.}}
\put(32.0,60.0){\circle*{1.}}
\put(3.2,54.0){\circle*{1.}}
\put(9.6,54.0){\circle*{1.}}
\put(16.0,54.0){\circle*{1.}}
\put(22.4,54.0){\circle*{1.}}
\put(28.800001,54.0){\circle*{1.}}
\put(0.0,48.0){\circle*{1.}}
\put(6.4,48.0){\circle*{1.}}
\put(12.8,48.0){\circle*{1.}}
\put(19.2,48.0){\circle*{1.}}
\put(25.6,48.0){\circle*{1.}}
\put(32.0,48.0){\circle*{1.}}
\put(3.2,42.0){\circle*{1.}}
\put(9.6,42.0){\circle*{1.}}
\put(16.0,42.0){\circle*{1.}}
\put(22.4,42.0){\circle*{1.}}
\put(28.800001,42.0){\circle*{6.8}}
\put(0.0,36.0){\circle*{1.}}
\put(6.4,36.0){\circle*{1.}}
\put(12.8,36.0){\circle*{1.}}
\put(19.2,36.0){\circle*{1.}}
\put(25.6,36.0){\circle*{1.}}
\put(32.0,36.0){\circle*{1.}}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(22.4,30.0){\circle*{1.}}
\put(28.800001,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{1.}}
\put(12.8,24.0){\circle*{1.}}
\put(19.2,24.0){\circle*{1.}}
\put(25.6,24.0){\circle*{1.}}
\put(32.0,24.0){\circle*{1.}}
\put(3.2,18.0){\circle*{1.}}
\put(9.6,18.0){\circle*{1.}}
\put(16.0,18.0){\circle*{1.}}
\put(22.4,18.0){\circle*{1.}}
\put(28.800001,18.0){\circle*{1.}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{1.}}
\put(19.2,12.0){\circle*{1.}}
\put(25.6,12.0){\circle*{1.}}
\put(32.0,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(22.4,6.0){\circle*{1.}}
\put(28.800001,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\put(19.2,0.0){\circle*{1.}}
\put(25.6,0.0){\circle*{1.}}
\put(32.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































































==> atex02/04.tex <==
\begin{picture}(32.0,60.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,60.0){\circle*{1.}}
\put(6.4,60.0){\circle*{1.}}
\put(12.8,60.0){\circle*{1.}}
\put(19.2,60.0){\circle*{1.}}
\put(25.6,60.0){\circle*{1.}}
\put(32.0,60.0){\circle*{1.}}
\put(3.2,54.0){\circle*{1.}}
\put(9.6,54.0){\circle*{1.}}
\put(16.0,54.0){\circle*{1.}}
\put(22.4,54.0){\circle*{1.}}
\put(28.800001,54.0){\circle*{1.}}
\put(0.0,48.0){\circle*{1.}}
\put(6.4,48.0){\circle*{1.}}
\put(12.8,48.0){\circle*{1.}}
\put(19.2,48.0){\circle*{1.}}
\put(25.6,48.0){\circle*{1.}}
\put(32.0,48.0){\circle*{1.}}
\put(3.2,42.0){\circle*{1.}}
\put(9.6,42.0){\circle*{1.}}
\put(16.0,42.0){\circle*{1.}}
\put(22.4,42.0){\circle*{1.}}
\put(28.800001,42.0){\circle*{1.}}
\put(0.0,36.0){\circle*{1.}}
\put(6.4,36.0){\circle*{1.}}
\put(12.8,36.0){\circle*{1.}}
\put(19.2,36.0){\circle*{1.}}
\put(25.6,36.0){\circle*{1.}}
\put(32.0,36.0){\circle*{1.}}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(22.4,30.0){\circle*{1.}}
\put(28.800001,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{1.}}
\put(12.8,24.0){\circle*{1.}}
\put(19.2,24.0){\circle*{1.}}
\put(25.6,24.0){\circle*{1.}}
\put(32.0,24.0){\circle*{1.}}
\put(3.2,18.0){\circle*{1.}}
\put(9.6,18.0){\circle*{1.}}
\put(16.0,18.0){\circle*{1.}}
\put(22.4,18.0){\circle*{1.}}
\put(28.800001,18.0){\circle*{1.}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{1.}}
\put(19.2,12.0){\circle*{1.}}
\put(25.6,12.0){\circle*{1.}}
\put(32.0,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(22.4,6.0){\circle*{1.}}
\put(28.800001,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\put(19.2,0.0){\circle*{1.}}
\put(25.6,0.0){\circle*{1.}}
\put(32.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































































==> atex02/05.tex <==
\begin{picture}(32.0,60.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,60.0){\circle*{1.}}
\put(6.4,60.0){\circle*{1.}}
\put(12.8,60.0){\circle*{1.}}
\put(19.2,60.0){\circle*{1.}}
\put(25.6,60.0){\circle*{1.}}
\put(32.0,60.0){\circle*{1.}}
\put(3.2,54.0){\circle*{1.}}
\put(9.6,54.0){\circle*{1.}}
\put(16.0,54.0){\circle*{1.}}
\put(22.4,54.0){\circle*{1.}}
\put(28.800001,54.0){\circle*{1.}}
\put(0.0,48.0){\circle*{1.}}
\put(6.4,48.0){\circle*{1.}}
\put(12.8,48.0){\circle*{1.}}
\put(19.2,48.0){\circle*{1.}}
\put(25.6,48.0){\circle*{1.}}
\put(32.0,48.0){\circle*{1.}}
\put(3.2,42.0){\circle*{1.}}
\put(9.6,42.0){\circle*{1.}}
\put(16.0,42.0){\circle*{1.}}
\put(22.4,42.0){\circle*{1.}}
\put(28.800001,42.0){\circle*{1.}}
\put(0.0,36.0){\circle*{1.}}
\put(6.4,36.0){\circle*{1.}}
\put(12.8,36.0){\circle*{1.}}
\put(19.2,36.0){\circle*{1.}}
\put(25.6,36.0){\circle*{1.}}
\put(32.0,36.0){\circle*{1.}}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(22.4,30.0){\circle*{1.}}
\put(28.800001,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{1.}}
\put(12.8,24.0){\circle*{1.}}
\put(19.2,24.0){\circle*{1.}}
\put(25.6,24.0){\circle*{1.}}
\put(32.0,24.0){\circle*{1.}}
\put(3.2,18.0){\circle*{1.}}
\put(9.6,18.0){\circle*{1.}}
\put(16.0,18.0){\circle*{1.}}
\put(22.4,18.0){\circle*{1.}}
\put(28.800001,18.0){\circle*{1.}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{1.}}
\put(19.2,12.0){\circle*{1.}}
\put(25.6,12.0){\circle*{1.}}
\put(32.0,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(22.4,6.0){\circle*{1.}}
\put(28.800001,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\put(19.2,0.0){\circle*{1.}}
\put(25.6,0.0){\circle*{1.}}
\put(32.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































































==> atex06/5.tex <==
\begin{picture}(32.0,60.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,60.0){\circle*{1.}}
\put(6.4,60.0){\circle*{1.}}
\put(12.8,60.0){\circle*{1.}}
\put(19.2,60.0){\circle*{1.}}
\put(25.6,60.0){\circle*{6.8}}
\put(32.0,60.0){\circle{6.8}}
\put(3.2,54.0){\circle*{1.}}
\put(9.6,54.0){\circle*{1.}}
\put(16.0,54.0){\circle*{1.}}
\put(22.4,54.0){\circle*{1.}}
\put(28.800001,54.0){\circle*{1.}}
\put(0.0,48.0){\circle*{1.}}
\put(6.4,48.0){\circle*{1.}}
\put(12.8,48.0){\circle*{1.}}
\put(19.2,48.0){\circle*{1.}}
\put(25.6,48.0){\circle*{1.}}
\put(32.0,48.0){\circle*{1.}}
\put(3.2,42.0){\circle*{1.}}
\put(9.6,42.0){\circle*{1.}}
\put(16.0,42.0){\circle*{1.}}
\put(22.4,42.0){\circle*{1.}}
\put(28.800001,42.0){\circle*{1.}}
\put(0.0,36.0){\circle*{1.}}
\put(6.4,36.0){\circle*{1.}}
\put(12.8,36.0){\circle*{1.}}
\put(19.2,36.0){\circle*{1.}}
\put(25.6,36.0){\circle*{1.}}
\put(32.0,36.0){\circle*{1.}}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(22.4,30.0){\circle*{1.}}
\put(28.800001,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{1.}}
\put(12.8,24.0){\circle*{1.}}
\put(19.2,24.0){\circle*{1.}}
\put(25.6,24.0){\circle*{1.}}
\put(32.0,24.0){\circle*{1.}}
\put(3.2,18.0){\circle*{1.}}
\put(9.6,18.0){\circle*{1.}}
\put(16.0,18.0){\circle*{1.}}
\put(22.4,18.0){\circle*{1.}}
\put(28.800001,18.0){\circle*{1.}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{1.}}
\put(19.2,12.0){\circle*{1.}}
\put(25.6,12.0){\circle*{1.}}
\put(32.0,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(22.4,6.0){\circle*{1.}}
\put(28.800001,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\put(19.2,0.0){\circle*{1.}}
\put(25.6,0.0){\circle*{1.}}
\put(32.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































































==> tex01/3.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{1.}}
\put(12.8,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{1.}}
\put(9.6,24.0){\circle*{1.}}
\put(16.0,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{1.}}
\put(6.4,18.0){\circle{6.8}}
\put(12.8,18.0){\circle*{1.}}
\put(3.2,12.0){\circle*{1.}}
\put(9.6,12.0){\circle*{6.8}}
\put(16.0,12.0){\circle*{6.8}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle{6.8}}
\put(12.8,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex01/4.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{1.}}
\put(12.8,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{1.}}
\put(9.6,24.0){\circle*{1.}}
\put(16.0,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{1.}}
\put(6.4,18.0){\circle*{1.}}
\put(12.8,18.0){\circle{6.8}}
\put(3.2,12.0){\circle*{6.8}}
\put(9.6,12.0){\circle*{6.8}}
\put(16.0,12.0){\circle*{1.}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle{6.8}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex01/5.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{1.}}
\put(12.8,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{1.}}
\put(9.6,24.0){\circle*{1.}}
\put(16.0,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{1.}}
\put(6.4,18.0){\circle{6.8}}
\put(12.8,18.0){\circle*{1.}}
\put(3.2,12.0){\circle*{1.}}
\put(9.6,12.0){\circle*{6.8}}
\put(16.0,12.0){\circle*{6.8}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle{6.8}}
\put(12.8,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex02/03.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle{6.8}}
\put(12.8,24.0){\circle*{1.}}
\put(3.2,18.0){\circle{6.8}}
\put(9.6,18.0){\circle{6.8}}
\put(16.0,18.0){\circle*{1.}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex02/04.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{6.8}}
\put(12.8,24.0){\circle*{1.}}
\put(3.2,18.0){\circle*{6.8}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle*{1.}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex02/05.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle{6.8}}
\put(12.8,24.0){\circle*{1.}}
\put(3.2,18.0){\circle{6.8}}
\put(9.6,18.0){\circle{6.8}}
\put(16.0,18.0){\circle*{1.}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex03/02.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{1.}}
\put(12.8,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{1.}}
\put(9.6,24.0){\circle*{1.}}
\put(16.0,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{1.}}
\put(6.4,18.0){\circle{6.8}}
\put(12.8,18.0){\circle*{6.8}}
\put(3.2,12.0){\circle*{1.}}
\put(9.6,12.0){\circle*{6.8}}
\put(16.0,12.0){\circle{6.8}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex03/03.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{1.}}
\put(12.8,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{1.}}
\put(9.6,24.0){\circle*{1.}}
\put(16.0,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{1.}}
\put(6.4,18.0){\circle{6.8}}
\put(12.8,18.0){\circle*{6.8}}
\put(3.2,12.0){\circle*{1.}}
\put(9.6,12.0){\circle*{6.8}}
\put(16.0,12.0){\circle{6.8}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex03/04.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{1.}}
\put(12.8,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{1.}}
\put(9.6,24.0){\circle*{1.}}
\put(16.0,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{1.}}
\put(6.4,18.0){\circle{6.8}}
\put(12.8,18.0){\circle*{6.8}}
\put(3.2,12.0){\circle*{1.}}
\put(9.6,12.0){\circle*{6.8}}
\put(16.0,12.0){\circle{6.8}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex03/05.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{1.}}
\put(12.8,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{1.}}
\put(9.6,24.0){\circle*{1.}}
\put(16.0,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{1.}}
\put(6.4,18.0){\circle{6.8}}
\put(12.8,18.0){\circle*{6.8}}
\put(3.2,12.0){\circle*{1.}}
\put(9.6,12.0){\circle*{6.8}}
\put(16.0,12.0){\circle{6.8}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex04/02.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{6.8}}
\put(12.8,24.0){\circle*{6.8}}
\put(3.2,18.0){\circle*{1.}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle{6.8}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex04/03.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{6.8}}
\put(12.8,24.0){\circle*{6.8}}
\put(3.2,18.0){\circle*{1.}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle{6.8}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex04/04.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{6.8}}
\put(12.8,24.0){\circle*{6.8}}
\put(3.2,18.0){\circle*{1.}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle{6.8}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex04/05.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{6.8}}
\put(12.8,24.0){\circle*{6.8}}
\put(3.2,18.0){\circle*{1.}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle{6.8}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex05/03.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{1.}}
\put(12.8,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{6.8}}
\put(9.6,24.0){\circle*{1.}}
\put(16.0,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{1.}}
\put(6.4,18.0){\circle*{6.8}}
\put(12.8,18.0){\circle{6.8}}
\put(3.2,12.0){\circle*{6.8}}
\put(9.6,12.0){\circle*{1.}}
\put(16.0,12.0){\circle*{1.}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex05/04.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{1.}}
\put(12.8,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{1.}}
\put(9.6,24.0){\circle*{6.8}}
\put(16.0,24.0){\circle*{1.}}
\put(0.0,18.0){\circle{6.8}}
\put(6.4,18.0){\circle*{6.8}}
\put(12.8,18.0){\circle*{1.}}
\put(3.2,12.0){\circle*{1.}}
\put(9.6,12.0){\circle*{6.8}}
\put(16.0,12.0){\circle*{1.}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex05/05.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{1.}}
\put(12.8,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{6.8}}
\put(9.6,24.0){\circle*{1.}}
\put(16.0,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{1.}}
\put(6.4,18.0){\circle*{6.8}}
\put(12.8,18.0){\circle{6.8}}
\put(3.2,12.0){\circle*{6.8}}
\put(9.6,12.0){\circle*{1.}}
\put(16.0,12.0){\circle*{1.}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex06/03.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{6.8}}
\put(12.8,24.0){\circle*{1.}}
\put(3.2,18.0){\circle*{1.}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle*{6.8}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{6.8}}
\put(12.8,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex06/04.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{1.}}
\put(12.8,24.0){\circle*{6.8}}
\put(3.2,18.0){\circle*{6.8}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle*{1.}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{6.8}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex06/05.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{6.8}}
\put(12.8,24.0){\circle*{1.}}
\put(3.2,18.0){\circle*{1.}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle*{6.8}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{6.8}}
\put(12.8,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex08/03.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{1.}}
\put(12.8,24.0){\circle{6.8}}
\put(3.2,18.0){\circle*{6.8}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle*{1.}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{6.8}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex08/04.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{6.8}}
\put(12.8,24.0){\circle*{1.}}
\put(3.2,18.0){\circle*{1.}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle*{6.8}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle{6.8}}
\put(12.8,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex08/05.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{1.}}
\put(12.8,24.0){\circle{6.8}}
\put(3.2,18.0){\circle*{6.8}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle*{1.}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{6.8}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex09/3.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle{6.8}}
\put(12.8,24.0){\circle*{1.}}
\put(3.2,18.0){\circle*{6.8}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle*{1.}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle{6.8}}
\put(12.8,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex09/4.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{6.8}}
\put(12.8,24.0){\circle*{1.}}
\put(3.2,18.0){\circle*{6.8}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle*{1.}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{6.8}}
\put(12.8,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex09/5.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{1.}}
\put(16.0,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle{6.8}}
\put(12.8,24.0){\circle*{1.}}
\put(3.2,18.0){\circle*{6.8}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle*{1.}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle{6.8}}
\put(12.8,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex10/3.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{1.}}
\put(12.8,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{6.8}}
\put(9.6,24.0){\circle{6.8}}
\put(16.0,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{6.8}}
\put(6.4,18.0){\circle*{1.}}
\put(12.8,18.0){\circle{6.8}}
\put(3.2,12.0){\circle*{6.8}}
\put(9.6,12.0){\circle*{6.8}}
\put(16.0,12.0){\circle*{1.}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex10/4.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{1.}}
\put(12.8,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{6.8}}
\put(9.6,24.0){\circle*{6.8}}
\put(16.0,24.0){\circle*{1.}}
\put(0.0,18.0){\circle{6.8}}
\put(6.4,18.0){\circle*{1.}}
\put(12.8,18.0){\circle*{6.8}}
\put(3.2,12.0){\circle{6.8}}
\put(9.6,12.0){\circle*{6.8}}
\put(16.0,12.0){\circle*{1.}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex10/5.tex <==
\begin{picture}(16.0,30.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{1.}}
\put(12.8,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{6.8}}
\put(9.6,24.0){\circle{6.8}}
\put(16.0,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{6.8}}
\put(6.4,18.0){\circle*{1.}}
\put(12.8,18.0){\circle{6.8}}
\put(3.2,12.0){\circle*{6.8}}
\put(9.6,12.0){\circle*{6.8}}
\put(16.0,12.0){\circle*{1.}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































==> tex12/03.tex <==
\begin{picture}(32.0,60.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,60.0){\circle*{1.}}
\put(6.4,60.0){\circle*{1.}}
\put(12.8,60.0){\circle*{1.}}
\put(19.2,60.0){\circle*{1.}}
\put(25.6,60.0){\circle*{1.}}
\put(32.0,60.0){\circle*{1.}}
\put(3.2,54.0){\circle*{1.}}
\put(9.6,54.0){\circle*{1.}}
\put(16.0,54.0){\circle*{1.}}
\put(22.4,54.0){\circle*{1.}}
\put(28.800001,54.0){\circle*{1.}}
\put(0.0,48.0){\circle*{1.}}
\put(6.4,48.0){\circle*{1.}}
\put(12.8,48.0){\circle*{1.}}
\put(19.2,48.0){\circle*{1.}}
\put(25.6,48.0){\circle*{1.}}
\put(32.0,48.0){\circle*{1.}}
\put(3.2,42.0){\circle*{1.}}
\put(9.6,42.0){\circle*{1.}}
\put(16.0,42.0){\circle*{6.8}}
\put(22.4,42.0){\circle*{6.8}}
\put(28.800001,42.0){\circle*{1.}}
\put(0.0,36.0){\circle*{1.}}
\put(6.4,36.0){\circle*{1.}}
\put(12.8,36.0){\circle*{6.8}}
\put(19.2,36.0){\circle*{1.}}
\put(25.6,36.0){\circle*{6.8}}
\put(32.0,36.0){\circle*{1.}}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{6.8}}
\put(16.0,30.0){\circle*{1.}}
\put(22.4,30.0){\circle*{6.8}}
\put(28.800001,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{6.8}}
\put(12.8,24.0){\circle*{1.}}
\put(19.2,24.0){\circle*{6.8}}
\put(25.6,24.0){\circle*{1.}}
\put(32.0,24.0){\circle*{1.}}
\put(3.2,18.0){\circle*{1.}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle*{6.8}}
\put(22.4,18.0){\circle*{1.}}
\put(28.800001,18.0){\circle*{1.}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{1.}}
\put(19.2,12.0){\circle*{1.}}
\put(25.6,12.0){\circle*{1.}}
\put(32.0,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(22.4,6.0){\circle*{1.}}
\put(28.800001,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\put(19.2,0.0){\circle*{1.}}
\put(25.6,0.0){\circle*{1.}}
\put(32.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































































==> tex12/04.tex <==
\begin{picture}(32.0,60.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,60.0){\circle*{1.}}
\put(6.4,60.0){\circle*{1.}}
\put(12.8,60.0){\circle*{1.}}
\put(19.2,60.0){\circle*{1.}}
\put(25.6,60.0){\circle*{1.}}
\put(32.0,60.0){\circle*{1.}}
\put(3.2,54.0){\circle*{1.}}
\put(9.6,54.0){\circle*{1.}}
\put(16.0,54.0){\circle*{1.}}
\put(22.4,54.0){\circle*{1.}}
\put(28.800001,54.0){\circle*{1.}}
\put(0.0,48.0){\circle*{1.}}
\put(6.4,48.0){\circle*{1.}}
\put(12.8,48.0){\circle*{1.}}
\put(19.2,48.0){\circle*{1.}}
\put(25.6,48.0){\circle*{1.}}
\put(32.0,48.0){\circle*{1.}}
\put(3.2,42.0){\circle*{1.}}
\put(9.6,42.0){\circle*{1.}}
\put(16.0,42.0){\circle*{6.8}}
\put(22.4,42.0){\circle*{6.8}}
\put(28.800001,42.0){\circle*{1.}}
\put(0.0,36.0){\circle*{1.}}
\put(6.4,36.0){\circle*{1.}}
\put(12.8,36.0){\circle*{6.8}}
\put(19.2,36.0){\circle*{1.}}
\put(25.6,36.0){\circle*{6.8}}
\put(32.0,36.0){\circle*{1.}}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{6.8}}
\put(16.0,30.0){\circle*{6.8}}
\put(22.4,30.0){\circle*{6.8}}
\put(28.800001,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{6.8}}
\put(12.8,24.0){\circle*{1.}}
\put(19.2,24.0){\circle*{6.8}}
\put(25.6,24.0){\circle*{1.}}
\put(32.0,24.0){\circle*{1.}}
\put(3.2,18.0){\circle*{1.}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle*{6.8}}
\put(22.4,18.0){\circle*{1.}}
\put(28.800001,18.0){\circle*{1.}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{1.}}
\put(19.2,12.0){\circle*{1.}}
\put(25.6,12.0){\circle*{1.}}
\put(32.0,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(22.4,6.0){\circle*{1.}}
\put(28.800001,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\put(19.2,0.0){\circle*{1.}}
\put(25.6,0.0){\circle*{1.}}
\put(32.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































































==> tex12/05.tex <==
\begin{picture}(32.0,60.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(0.0,60.0){\circle*{1.}}
\put(6.4,60.0){\circle*{1.}}
\put(12.8,60.0){\circle*{1.}}
\put(19.2,60.0){\circle*{1.}}
\put(25.6,60.0){\circle*{1.}}
\put(32.0,60.0){\circle*{1.}}
\put(3.2,54.0){\circle*{1.}}
\put(9.6,54.0){\circle*{1.}}
\put(16.0,54.0){\circle*{1.}}
\put(22.4,54.0){\circle*{1.}}
\put(28.800001,54.0){\circle*{1.}}
\put(0.0,48.0){\circle*{1.}}
\put(6.4,48.0){\circle*{1.}}
\put(12.8,48.0){\circle*{1.}}
\put(19.2,48.0){\circle*{1.}}
\put(25.6,48.0){\circle*{1.}}
\put(32.0,48.0){\circle*{1.}}
\put(3.2,42.0){\circle*{1.}}
\put(9.6,42.0){\circle*{1.}}
\put(16.0,42.0){\circle*{6.8}}
\put(22.4,42.0){\circle*{6.8}}
\put(28.800001,42.0){\circle*{1.}}
\put(0.0,36.0){\circle*{1.}}
\put(6.4,36.0){\circle*{1.}}
\put(12.8,36.0){\circle*{6.8}}
\put(19.2,36.0){\circle*{1.}}
\put(25.6,36.0){\circle*{6.8}}
\put(32.0,36.0){\circle*{1.}}
\put(3.2,30.0){\circle*{1.}}
\put(9.6,30.0){\circle*{6.8}}
\put(16.0,30.0){\circle*{1.}}
\put(22.4,30.0){\circle*{6.8}}
\put(28.800001,30.0){\circle*{1.}}
\put(0.0,24.0){\circle*{1.}}
\put(6.4,24.0){\circle*{6.8}}
\put(12.8,24.0){\circle*{1.}}
\put(19.2,24.0){\circle*{6.8}}
\put(25.6,24.0){\circle*{1.}}
\put(32.0,24.0){\circle*{1.}}
\put(3.2,18.0){\circle*{1.}}
\put(9.6,18.0){\circle*{6.8}}
\put(16.0,18.0){\circle*{6.8}}
\put(22.4,18.0){\circle*{1.}}
\put(28.800001,18.0){\circle*{1.}}
\put(0.0,12.0){\circle*{1.}}
\put(6.4,12.0){\circle*{1.}}
\put(12.8,12.0){\circle*{1.}}
\put(19.2,12.0){\circle*{1.}}
\put(25.6,12.0){\circle*{1.}}
\put(32.0,12.0){\circle*{1.}}
\put(3.2,6.0){\circle*{1.}}
\put(9.6,6.0){\circle*{1.}}
\put(16.0,6.0){\circle*{1.}}
\put(22.4,6.0){\circle*{1.}}
\put(28.800001,6.0){\circle*{1.}}
\put(0.0,0.0){\circle*{1.}}
\put(6.4,0.0){\circle*{1.}}
\put(12.8,0.0){\circle*{1.}}
\put(19.2,0.0){\circle*{1.}}
\put(25.6,0.0){\circle*{1.}}
\put(32.0,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































































==> tex13/04.tex <==
\begin{picture}(32.0,60.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,60.0){\circle*{1.}}
\put(9.6,60.0){\circle*{1.}}
\put(16.0,60.0){\circle*{1.}}
\put(22.4,60.0){\circle*{1.}}
\put(28.800001,60.0){\circle*{1.}}
\put(0.0,54.0){\circle*{1.}}
\put(6.4,54.0){\circle*{1.}}
\put(12.8,54.0){\circle*{1.}}
\put(19.2,54.0){\circle*{1.}}
\put(25.6,54.0){\circle*{1.}}
\put(32.0,54.0){\circle*{1.}}
\put(3.2,48.0){\circle*{1.}}
\put(9.6,48.0){\circle*{1.}}
\put(16.0,48.0){\circle*{1.}}
\put(22.4,48.0){\circle*{1.}}
\put(28.800001,48.0){\circle*{1.}}
\put(0.0,42.0){\circle*{1.}}
\put(6.4,42.0){\circle*{1.}}
\put(12.8,42.0){\circle*{1.}}
\put(19.2,42.0){\circle*{1.}}
\put(25.6,42.0){\circle*{1.}}
\put(32.0,42.0){\circle*{1.}}
\put(3.2,36.0){\circle*{1.}}
\put(9.6,36.0){\circle{6.8}}
\put(16.0,36.0){\circle*{6.8}}
\put(22.4,36.0){\circle*{6.8}}
\put(28.800001,36.0){\circle*{1.}}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{6.8}}
\put(12.8,30.0){\circle*{1.}}
\put(19.2,30.0){\circle*{1.}}
\put(25.6,30.0){\circle*{6.8}}
\put(32.0,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{1.}}
\put(9.6,24.0){\circle{6.8}}
\put(16.0,24.0){\circle*{6.8}}
\put(22.4,24.0){\circle*{6.8}}
\put(28.800001,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{1.}}
\put(6.4,18.0){\circle*{1.}}
\put(12.8,18.0){\circle*{1.}}
\put(19.2,18.0){\circle*{1.}}
\put(25.6,18.0){\circle*{1.}}
\put(32.0,18.0){\circle*{1.}}
\put(3.2,12.0){\circle*{1.}}
\put(9.6,12.0){\circle*{1.}}
\put(16.0,12.0){\circle*{1.}}
\put(22.4,12.0){\circle*{1.}}
\put(28.800001,12.0){\circle*{1.}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(19.2,6.0){\circle*{1.}}
\put(25.6,6.0){\circle*{1.}}
\put(32.0,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\put(22.4,0.0){\circle*{1.}}
\put(28.800001,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}









































































































































==> tex13/05.tex <==
\begin{picture}(32.0,60.0)
\begin{footnotesize}
\linethickness{0.800000pt}
\put(3.2,60.0){\circle*{1.}}
\put(9.6,60.0){\circle*{1.}}
\put(16.0,60.0){\circle*{1.}}
\put(22.4,60.0){\circle*{1.}}
\put(28.800001,60.0){\circle*{1.}}
\put(0.0,54.0){\circle*{1.}}
\put(6.4,54.0){\circle*{1.}}
\put(12.8,54.0){\circle*{1.}}
\put(19.2,54.0){\circle*{1.}}
\put(25.6,54.0){\circle*{1.}}
\put(32.0,54.0){\circle*{1.}}
\put(3.2,48.0){\circle*{1.}}
\put(9.6,48.0){\circle*{1.}}
\put(16.0,48.0){\circle*{1.}}
\put(22.4,48.0){\circle*{1.}}
\put(28.800001,48.0){\circle*{1.}}
\put(0.0,42.0){\circle*{1.}}
\put(6.4,42.0){\circle*{1.}}
\put(12.8,42.0){\circle*{1.}}
\put(19.2,42.0){\circle*{1.}}
\put(25.6,42.0){\circle*{1.}}
\put(32.0,42.0){\circle*{1.}}
\put(3.2,36.0){\circle*{1.}}
\put(9.6,36.0){\circle{6.8}}
\put(16.0,36.0){\circle{6.8}}
\put(22.4,36.0){\circle*{6.8}}
\put(28.800001,36.0){\circle*{1.}}
\put(0.0,30.0){\circle*{1.}}
\put(6.4,30.0){\circle*{6.8}}
\put(12.8,30.0){\circle*{1.}}
\put(19.2,30.0){\circle*{1.}}
\put(25.6,30.0){\circle*{6.8}}
\put(32.0,30.0){\circle*{1.}}
\put(3.2,24.0){\circle*{1.}}
\put(9.6,24.0){\circle{6.8}}
\put(16.0,24.0){\circle{6.8}}
\put(22.4,24.0){\circle*{6.8}}
\put(28.800001,24.0){\circle*{1.}}
\put(0.0,18.0){\circle*{1.}}
\put(6.4,18.0){\circle*{1.}}
\put(12.8,18.0){\circle*{1.}}
\put(19.2,18.0){\circle*{1.}}
\put(25.6,18.0){\circle*{1.}}
\put(32.0,18.0){\circle*{1.}}
\put(3.2,12.0){\circle*{1.}}
\put(9.6,12.0){\circle*{1.}}
\put(16.0,12.0){\circle*{1.}}
\put(22.4,12.0){\circle*{1.}}
\put(28.800001,12.0){\circle*{1.}}
\put(0.0,6.0){\circle*{1.}}
\put(6.4,6.0){\circle*{1.}}
\put(12.8,6.0){\circle*{1.}}
\put(19.2,6.0){\circle*{1.}}
\put(25.6,6.0){\circle*{1.}}
\put(32.0,6.0){\circle*{1.}}
\put(3.2,0.0){\circle*{1.}}
\put(9.6,0.0){\circle*{1.}}
\put(16.0,0.0){\circle*{1.}}
\put(22.4,0.0){\circle*{1.}}
\put(28.800001,0.0){\circle*{1.}}
\end{footnotesize}
\end{picture}








































































































































